The Power of Connection: Leveraging Network Analysis to Advance Receivable Financing

Receivable financing is the process whereby cash is advanced to firms against receivables their customers have yet to pay: a receivable can be sold to a funder, which immediately gives the firm cash in return for a small percentage of the receivable amount as a fee. Receivable financing has been traditionally handled in a centralized way, where every request is processed by the funder individually and independently of one another. In this work we propose a novel, network-based approach to receivable financing, which enables customers of the same funder to autonomously pay each other as much as possible, and gives benefits to both the funder (reduced cash anticipation and exposure risk) and its customers (smaller fees and lightweight service establishment). Our main contributions consist in providing a principled formulation of the network-based receivable-settlement strategy, and showing how to achieve all algorithmic challenges posed by the design of this strategy. We formulate network-based receivable financing as a novel combinatorial-optimization problem on a multigraph of receivables. We show that the problem is NP-hard, and devise an exact branch-and-bound algorithm, as well as algorithms to efficiently find effective approximate solutions. Our more efficient algorithms are based on cycle enumeration and selection, and exploit a theoretical characterization in terms of a knapsack problem, as well as a refining strategy that properly adds paths between cycles. We also investigate the real-world issue of avoiding temporary violations of the problem constraints, and design methods for handling it. An extensive experimental evaluation is performed on real receivable data. Results attest the good performance of our methods.

==> deployment.tex <==
%!TEX root = balance_tnse2019_revision.tex
\section{Way to deployment}
\label{sec:deployment}

The deployment of the \balance platform is currently in progress.
The process is expected to end in a few months.
Then, the pilot phase of \balance as a banking product will start, during which the product will be tested by a (limited) number of ad-hoc-selected customers.
The algorithm for network-based invoice settlement ultimately proposed in this work (Algorithm~\ref{alg:hybridalg}) is implemented in a software module that constitutes the \emph{core} of a more general architecture.
While being non-trivial as it has to handle all the technical aspects of system deployment at an industrial level, the architecture behind the \balance platform remains pretty standard.
For this reason, describing the architecture in detail is beyond the scope of this work.
%: here we focus on the part that is more challenging and appealing from a research point of view, i.e.,   
Here we just mention that, apart from the invoice-settlement core module, the architecture includes a number of standard modules such as data fetcher, preprocessor, recovery manager, and frontend, which have been already developed and are currently being tested.
The only module whose design is to some extent challenging is the so-called \emph{money-transfer executor}, which is responsible for the ultimate integration of the \balance platform within the in-house systems of the \unicredit bank.
This module is mainly devoted to interact with the \unicredit bank-account management system in order to have the money of every settled invoice transferred from the debtor's account to the creditor's account.
A technical challenge of this interaction is that,
to properly settle a set of invoices, it may be needed that the balance of the bank account of some customers \emph{temporarily} becomes smaller than the $floor$ allowed for those customers.
Even if this overdraft lasts at most a few milliseconds, to be handled properly it requires ad-hoc money-transfer mechanisms (standard bank transfers, e.g., cannot be used) and robust roll-back methodologies (in the event that something goes wrong).
Such a module is currently under development and represents the main to-do before getting to the final deployment of the platform.

==> experiments_compact.tex <==
%!TEX root = balance_arxiv.tex
\section{Experiments}
\label{sec:experiments}

\begin{table*}[t]
\vspace{-4mm}
\begin{center}
\vspace{-0mm}
{
\caption{{\footnotesize \label{tbl:graph-stats} Size of the input \bmultigraph{s} extracted from the real datasets considered in the experiments (algorithm: \bsalg).}} 
\vspace{-0.2cm}
\scriptsize
%\begin{tabular}{cl|@{~~}||@{~~} l@{~~} ||@{~~}S[table-format=5]@{~~}S[table-format=6]@{~~} |@{~~} S[table-format=5]@{~~} S[table-format=6] @{~~} || @{~~} S[table-format=5]@{~~} S[table-format=6] @{~~} | @{~~} S[table-format=5]@{~~} S[table-format=6]@{~~} ||@{~~} S[table-format=6]@{~~} S[table-format=6]@{~~} |@{~~} S[table-format=6]@{~~} S[table-format=6]@{~~}} 
%dataset & \multicolumn{1}{l||@{~~}}{\multirow{3}{*}{\textbf{Time Span}}} & \multicolumn{1}{c||@{~~}}{\multirow{3}{*}{\textbf{Size}}}  & \multicolumn{4}{c||@{~~}}{\textbf{Worst Scenario}} & \multicolumn{4}{c||@{~~}}{\textbf{Normal Scenario}} & \multicolumn{4}{c@{~~}}{\textbf{Best Scenario}} \\
%& & & \multicolumn{2}{c|@{~~}}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c||@{~~}}{\textbf{CAP $= \infty$}} & \multicolumn{2}{c|@{~~}}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c||@{~~}}{\textbf{CAP $= \infty$}} & \multicolumn{2}{c|@{~~}}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c@{~~~}}{\textbf{CAP $= \infty$}} \\
%& & &  \textbf{Avg} & \textbf{Max} &  \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max} & \textbf{Avg} & \textbf{Max }\\ 
\begin{tabular}{@{}c@{ }@{ }c@{ }||c@{ }||S[table-format=5]@{~~}S[table-format=6]|S[table-format=5]@{~~}S[table-format=6]||S[table-format=5]@{~~}S[table-format=6]|S[table-format=5]@{~~}S[table-format=6]||S[table-format=6]@{~~}S[table-format=6]|S[table-format=6]@{~~}S[table-format=6]@{}} 
\multirow{3}{*}{\textbf{dataset}} & \multicolumn{1}{c||}{\multirow{3}{*}{\textbf{span}}} & \multicolumn{1}{c||}{\multirow{3}{*}{\textbf{size}}}  & \multicolumn{4}{c||}{\textbf{Worst scenario}} & \multicolumn{4}{c||}{\textbf{Normal scenario}} & \multicolumn{4}{c}{\textbf{Best scenario}} \\
 & & & \multicolumn{2}{c|}{\textbf{CAP} $< \infty$} & \multicolumn{2}{c||}{\textbf{CAP} $= \infty$} & \multicolumn{2}{c|}{\textbf{CAP} $< \infty$} & \multicolumn{2}{c||}{\textbf{CAP} $= \infty$} & \multicolumn{2}{c|}{\textbf{CAP} $< \infty$} & \multicolumn{2}{c}{\textbf{CAP} $= \infty$}\\
 & & & \textbf{avg} & \textbf{max} & \textbf{avg} & \textbf{max}  & \textbf{avg} & \textbf{max} & \textbf{avg} & \textbf{max} & \textbf{avg} & \textbf{max} & \textbf{avg} & \textbf{max}\\
\hline
\multirow{2}{*}{\firstlog} &  {\multirow{2}{*}{\textbf{2015/16}}}  & \textbf{\#nodes} &  40810  &  58390 &  40810 &  58380  &  62890 & 82930  &  62870 &  82900  &   80260  &  97400   &  80230 &   97380 \\ 
& & \textbf{\#arcs} &  41720 &   69270  &  41670  &   69180   & 76490  &  116000  &  76310  & 115600   &  111100 & 149300  &  110700 &  148500 \\ 
\hline 
\multirow{2}{*}{\secondlog} &  {\multirow{2}{*}{\textbf{2017/18}}}  & \textbf{\#nodes} &   50563  & 77323   &  50548   &  77280  & 77134  & 105671   &  77082  & 105627 & 97888 & 121274 &  97789   & 121244   \\
& & \textbf{\#arcs}  & 51708   &  132944  &  51600 & 132786  &  92560 & 215913 &  92025  & 215078 & 132564  & 278246 & 131325  & 276497 \\
\end{tabular}}
\end{center}
\vspace{-5mm}
\end{table*}

%\subsection{Datasets and evaluation settings}
\spara{Datasets.}
We tested the performance of our algorithms on two \emph{real datasets} provided by \unicredit, a noteworthy pan-European commercial bank. 
Each dataset consists of a random sample of the receivable log of the bank, spanning a time interval of one year, in 2015/16 (\firstlog) and 2017/18 (\secondlog), respectively.
Each dataset includes roughly 5M receivables and 400K (anonymized) customers.
%: the former, dubbed \firstlog, dates back to \mbox{2015-16}, while the latter, named \secondlog, spans \mbox{2017-18}. 
%Table~\ref{tbl:graph-stats} reports statistics on the \bmultigraph{s} extracted from the two datasets. 
%The sample consists of $5\,413\,375$  receivables and  $369\,479$ (anonymized) customers, spanning one year in \mbox{2015-16}.  --> WE DO NOT HAVE THIS DATA FOR THE SECOND DATASET, CHECK IF WE CAN RETRIEVE THAT 

%The invoices were randomly sampled from the request database of a European country, and anonymized.
%Given that the input data was not provided with node attributes, we simulated the values of the \bala, the \ub and \lb of each client based on customer-specific statistics that we computed on a training prefix of three months of data.

\spara{Customers' attributes.} 
We set customers' attributes based on statistics computed on a training prefix of 3 months.

As far as the initial actual balance $\bala(u)$ of a customer $u$, we computed the difference between the total amount of her passive receivables and the total amount of her active receivables;
we considered the days were such a difference was negative, and ultimately set $\bala(u)$ as the average of the absolute values of such negative daily differences.
The rationale is that in those days the customer would have needed extra liquidity with respect to the amount cashable from incoming receivables, to handle the payment of the receivables in which she was listed as payer.
%The rationale was to choose a value that would allow the customer to handle her typical payment needs based on her behavior observed in the training data. 
Assuming that in reality customers would try this new service with a limited initial cash deposit, we also imposed a hard upper bound of $50K$ euros for the initial \bala of every customer.
%Because we did not want any client to start the game with an excessive cash availability in her account, we actually did not allow any customer to have 
%an initial balance greater than $50K$ euros: thus, in the cases where the above rule was leading to a value exceeding the threshold, we corrected it to $50K$.
%For clients with no negative differences between amount received and amount payed in the training data, 
%In the case of a customer for whom we never observe in the training data days where the difference between the amount received is lower than the amount payed, 
%i.e., if a client never seems to need in the training phase, extra cash with respect to the liquidity she cashes from invoices where she is the beneficiary, 
%we set the initial \bala to $0$.

As for the $\ub$, we considered: ($i$)  finite $\ub$, equal to the average amount a customer received in the training data (customers with no payments in the training interval got a default $\ub$ equal to the average $\ub$ of all other customers); and ($ii$) $\ub = \infty$, where we allowed all accounts to grow arbitrarily.
%
Finally, we set $\lb(u) = 0$, for each customer $u$.

%\noindent\textbf{Invoice lifetime.} 
%For every invoice $I \in \mathcal{I}$, we considered $\lifetime(I)$ 
%%is the maximum time that $I$ is allowed to last inside \balance. 
%%Our commissioner institution intends to propose to its clients to keep an invoice in the platform for a short time, after which they may turn to traditional factoring if the invoice has not been settled successfully yet.
%%Given that the tool is intended to replace the standard invoice factoring mechanism of our commissioner institution, 
%%their business proposal to the users is to load and keep an invoice in this new tool for a small time, 
%%after which, in the case the tool has not been able to successfully factor that invoice, the customer is guaranteed access to the traditional factoring service. 
%%For the above reasons, the idea is that the lifetime of an invoice in our system should correspond to a pretty limited time intervals. 
%%We considered values 
%of 5, 10, and 15 days. 

\smallskip
\noindent\textbf{Simulation.}
%Varying all parameters as described above, 
We defined 6 simulation settings:
\vspace{-0mm}
\begin{smallenumerate}
\item \emph{Finite CAP.} Let $fcap(u)$ be the finite value of the $\ub$ of a  \mbox{customer $u$ computed as above. We~considered~3~scenarios}:
\vspace{-3mm}
\begin{smallitemize}
\item \emph{\!\!Worst:} $\lifetime(R) \!= \!5, \forall R \!\in\! \mathcal{R};  \ub(u) \!=\! fcap(u), \!\forall u \!\in\! \mathcal{U}$;
\item \mbox{\emph{\!\!Normal:} $\lifetime(R) \!=\! 10, \forall R \!\in\! \mathcal{R};  \ub(u) \!=\! 2fcap(u), \!\forall u \!\in\! \mathcal{U}$;}
\item \emph{\!\!Best:} $\lifetime(R) \!=\! 15, \forall R \!\in\! \mathcal{R};   \ub(u) \!=\! 3fcap(u), \!\forall u \!\in\! \mathcal{U}$;
\end{smallitemize}
\vspace{1mm}
\item \emph{CAP $= \infty$.} We considered \emph{Worst}, \emph{Normal}, and  \emph{Best} scenarios here too, with \lifetime values equal to  the corresponding 
finite-CAP cases, but we set $\ub(u) = \infty$, $\forall u \in \mathcal{U}$.
\iffalse
\begin{smallitemize}
\vspace{1mm}
\item \emph{Worst:} $\lifetime(I) = 5 \mbox{ }, \forall I \in \mathcal{I}, \ \ \ub(u) = \infty \mbox{ }, \forall u \in \mathcal{U}$;
\item \emph{Normal:} $\lifetime(I) = 10 \mbox{ }, \forall I \in \mathcal{I}, \ \ \ub(u) = \infty \mbox{ }, \forall u \in \mathcal{U}$;
\item \emph{Best:} $\lifetime(I) = 15 \mbox{ }, \forall I \in \mathcal{I}, \ \ \ub(u) = \infty \mbox{ }, \forall u \in \mathcal{U}$;
\end{smallitemize}
\fi
\end{smallenumerate}
\vspace{-0mm}
%We tested the behavior of our algorithms on the whole dataset, except for the training prefix.
Such settings identify different sets of valid receivables for a day, thus yielding different input multigraphs.
Table~\ref{tbl:graph-stats} reports on the sizes of those multigraphs.
%More complex scenarios clearly lead to larger graphs. 
%Conversely,  as the $\ub$ goes from $<\!\!\infty$ to  $\infty$ (in the same scenario), graphs get smaller. 
%This is motivated as $\ub\!<\!\infty$ represents a tighter constraint for receivable settlement, i.e., more receivables not settled any day which will be included in the input graph of the next day.

%We divided the experimental assessment of our algorithms in two parts. First, we focused on evaluating the performance of the algorithms based on cycle selection, whilst in the second phase we assessed the contribution of adding paths between cycles. 

\spara{Assessment criteria.}
We assess the performance of the algorithms by measuring the total amount of the receivables that an algorithm selects for settlement.
This metric provides direct evidence of the benefits for both the funder and the customers: the greater the amount, the less liquidity the funder has to anticipate, and the larger the saving for customers due to the reduced fees of the network-based~service.

\spara{Parameters.}
Unless otherwise specified, all experiments refer to $\maxcyclelength=15$ (cycle-enumeration-based algorithm), $H=20$ (\bsalg), and  $K=1\,000$ (\bsalg and \hybridalg).

\spara{Testing environment.}
All algorithms were implemented in \textsf{Scala} (v. 2.12).
Experiments were run on an i9 Intel 7900x 3.3GHz, 128GB RAM machine.
%(which we limited to 64GB RAM).
%Experiments in Table~\ref{table:scalability} were run on an i9 Intel 7900x 3.3GHz, 128GB RAM machine, which we limited to 60GB in our tests.
%All other experiments were run on a commodity laptop equipped with an Intel Core i7 CPU at 2.8GHz and 16GB RAM.

%\begin{table*}[t]
%\vspace{-2mm}
%\begin{center}{
%\caption{\footnotesize \label{tbl:baseline} Experimental results: proposed \hybridalgp vs. \rfbaseline baseline.}
%\vspace{-0.2cm}
%\scriptsize
%\begin{tabular}{c  | c || c  | S[table-format=9] |  S[table-format=9] S[table-format=4.1]  || c  | S[table-format=9]   | S[table-format=9] S[table-format=4.1]} 
%\multicolumn{1}{c|}{\textbf{quarter}} & \multicolumn{1}{c||}{\textbf{scenario}} & \multicolumn{1}{c}{\textbf{cap}} & \multicolumn{1}{c}{\textbf{\hybridalg}} & \multicolumn{2}{c||}{\textbf{\rfbaseline}} &   \multicolumn{1}{c}{\textbf{cap}} & \multicolumn{1}{c}{\textbf{\hybridalg}} & \multicolumn{2}{c}{\textbf{\rfbaseline}} \\
%\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{\textbf{amount}}  & \multicolumn{1}{c}{\textbf{amount}} &  \multicolumn{1}{c||}{\textbf{\% gain}} & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{\textbf{amount}}  & \multicolumn{1}{c}{\textbf{amount}} &  \multicolumn{1}{c}{\textbf{\% gain}} \\
%\hline
% $Q17_1$ & {\multirow{4}{*}{\textbf{W}}} &  {\multirow{12}{*}{\textbf{$<\!\!\infty$}}}  & 208452169 &  75871408 &  -63.6 & {\multirow{12}{*}{\textbf{$\infty$}}}  & 250919555 & 75871408  & -69.76  \\
% $Q17_2$ &  &  & 133998727 & 28759273 &  -78.53 & & 374766629 & 28759273  &  -92.32\\
% $Q17_3$ &  &  & 250919555 &  57472835 & -77.1 &  & 300021017 & 57472835 & -80.1 \\
% $Q17_4$ &  & & 435864820 & 128409243 &  -70.53 &  & 516434249 & 128409243 & -75.1 \\
%\cline{1-2}\cline{4-6}\cline{8-10}
%%\hline
%$Q17_1$ & {\multirow{4}{*}{\textbf{N}}} &  & 100052350 &  0 & -100  & & 395904601 & 0 & -100 \\
%$Q17_2$ & &  & 210803336 &  0 &  -100 &  & 555117105 &  0 & -100 \\
%$Q17_3$ &  & &  181024199 & 0 & -100 &  & 471313548 & 0 & -100 \\
%$Q17_4$ & & & 405407829 & 68940677 & -83 &  & 679395059 & 189533414 & -72.1 \\
%\cline{1-2}\cline{4-6}\cline{8-10}
% %\hline
% $Q17_1$  & {\multirow{4}{*}{\textbf{B}}} &  & 128172168  &  0 & -100 &  & 552458593 & 0 & -100 \\
% $Q17_2$  &  &   & 223972720 & 0 &  -100 & & 699245106 & 0 & -100 \\
% $Q17_3$  &  & & 138227899 & 0 &-100 &  & 544101823 & 0 & -100 \\
% $Q17_4$  &  &  & 380133762 & 0 & -100 &  & 907115932 & 120592737 & -86.7 \\
%\end{tabular}}
%\end{center}
%\vspace{-2mm}
%\end{table*}


\begin{table}[t]
%\vspace{2mm}
%\vspace{0mm}
\begin{center}{
\caption{\footnotesize \label{tbl:baseline} Proposed \hybridalg algorithm vs. \rfbaseline baseline.}
\vspace{-0.2cm}
\scriptsize
\begin{tabular}{c  | c || c  | S[table-format=9] |  S[table-format=9] S[table-format=4.1] } 
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{quarter}}} & \multicolumn{1}{c||}{\multirow{2}{*}{\textbf{scenario}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{cap}}} & \multicolumn{1}{c|}{\textbf{\hybridalg}} & \multicolumn{2}{c}{\textbf{\rfbaseline}}  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} &\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\textbf{amount}}  & \multicolumn{1}{c}{\textbf{amount}} &  \multicolumn{1}{c}{\textbf{\%gain}} \\
\hline
 $Q17_1$ & {\multirow{4}{*}{\textbf{W}}} &  {\multirow{12}{*}{\textbf{$<\!\!\infty$}}}  & 208452169 &  75871408 &  -63.6  \\
 $Q17_2$ &  &  & 133998727 & 28759273 &  -78.53 \\
 $Q17_3$ &  &  & 250919555 &  57472835 & -77.1 \\
 $Q17_4$ &  & & 435864820 & 128409243 &  -70.53 \\
\cline{1-2}\cline{4-6}
%\hline
$Q17_1$ & {\multirow{4}{*}{\textbf{N}}} &  & 100052350 &  0 & -100   \\
$Q17_2$ & &  & 210803336 &  0 &  -100  \\
$Q17_3$ &  & &  181024199 & 0 & -100  \\
$Q17_4$ & & & 405407829 & 68940677 & -83  \\
\cline{1-2}\cline{4-6}
 %\hline
 $Q17_1$  & {\multirow{4}{*}{\textbf{B}}} &  & 128172168  &  0 & -100  \\
 $Q17_2$  &  &   & 223972720 & 0 &  -100  \\
 $Q17_3$  &  & & 138227899 & 0 &-100  \\
 $Q17_4$  &  &  & 380133762 & 0 & -100  \\
 \hline
 \hline
 $Q17_1$ & {\multirow{4}{*}{\textbf{W}}} &   {\multirow{12}{*}{\textbf{$\infty$}}}  & 250919555 & 75871408  & -69.76  \\
 $Q17_2$ &  &  & 374766629 & 28759273  &  -92.32\\
 $Q17_3$ &  &  & 300021017 & 57472835 & -80.1 \\
 $Q17_4$ &  & & 516434249 & 128409243 & -75.1 \\
\cline{1-2}\cline{4-6}
%\hline
$Q17_1$ & {\multirow{4}{*}{\textbf{N}}} &  & 395904601 & 0 & -100 \\
$Q17_2$ & &  & 555117105 &  0 & -100 \\
$Q17_3$ &  & & 471313548 & 0 & -100 \\
$Q17_4$ & & & 679395059 & 189533414 & -72.1 \\
\cline{1-2}\cline{4-6}
 %\hline
 $Q17_1$  & {\multirow{4}{*}{\textbf{B}}} &  & 552458593 & 0 & -100 \\
 $Q17_2$  &  &   & 699245106 & 0 & -100 \\
 $Q17_3$  &  & & 544101823 & 0 & -100 \\
 $Q17_4$  &  &  & 907115932 & 120592737 & -86.7 \\
\end{tabular}}
\end{center}
%\vspace{-3mm}
\vspace{-5mm}
\end{table}


\vspace{1mm}
\subsection{Results}

\vspace{1mm}
\spara{Comparison against a baseline.}
%Observe that we do not have external baselines to employ, as this is (to the best of our knowledge) the first attempt to exploit the receivable network to optimize RF.
%Whilst we are not aware of an external method suitable to be considered as a baseline, we defined a possible baseline for our \hybridalg algorithm as follows.
Whilst we are not aware of any external method, as this is (to the best of our knowledge) the first attempt to exploit the receivable network to optimize RF, we defined a possible baseline for the proposed \hybridalg algorithm (Algorithm~\ref{alg:hybridalg}) as follows.
%
We start from a solution $\E^* = \E$ composed of all the arcs of the input multigraph, and, as long as $\E^*$ violates one of the two constraints of Problem~\ref{problem:balancestatic}, we iteratively:
($i$) remove arcs from $\E^*$ in non-decreasing amount order, until Problem~\ref{problem:balancestatic}'s Constraint~(\ref{eq:prob1constraint1}) is satisfied; 
($ii$) extract the $(1,1)$-core from the subgraph induced by $\E^*$ (to satisfy Problem~\ref{problem:balancestatic}'s Consraint~(\ref{eq:prob1constraint2})). 
%We dub this baseline \rfbaseline. 
In Table~\ref{tbl:baseline} we compare this baseline, dubbed \rfbaseline, and \hybridalg on the \secondlog dataset.
We split the dataset into 3-month periods, to have a better understanding of the performance on a quarterly basis, 
and speed up the evaluation by parallelizing on different quarters.
%(divided in quarters as in the previous experiments). 
The main observation here is that the baseline achieves a consistent loss between $70\%$ and $100\%$ against \hybridalg in all quarters, and for all scenarios: this confirms the strength of the proposed algorithm.

\vspace{1mm}
\spara{Comparison among methods of this work.}
In our second experiment we assessed the proposed \hybridalg with respect to the other (simpler) methods devised in this work:
($i$) the  greedy-cycle-selection \johnson algorithm (Algorithm~\ref{alg:johnson}), and the beam-search \bsalg algorithm (Algorithm~\ref{alg:bsalg}).
As far as the exact \bbalg (Algorithm~\ref{alg:staticbalanceBB}), clearly it could not afford the sizes of our \bmultigraph{s}.
However, recall that \bbalg is part of \hybridalg, where it is run on the smaller connected components: an idea of its performance thus comes from the comparison  \hybridalg vs. \bsalg. This evaluation was ran on the  \firstlog dataset (divided in quarters as above).
%and all experiments refer to $\maxcyclelength=15$ (cycle-enumeration-based algorithm), $H=20$ (\bsalg), and  $K=1\,000$ (\bsalg and \hybridalg).
%Observe that we do not have external baselines to employ, as this is (to the best of our knowledge) the first attempt to exploit the receivable network to optimize RF.
For each scenario/quarter pair, we report (Table \ref{tbl:experimental-results}): total amount (euros) of the settled receivables, 
per-day running time (seconds) averaged on all the days in the quarter, total number of settled receivables, number of distinct customers in a daily solution, and percentage gain of the  \hybridalg's amount over the competitors.

% Comments about gain in amount
\hybridalg outperforms both competitors in terms of settled amount.
In the finite-cap, worst scenario,
the avg and max gain of \hybridalg over \johnson is $150\%$ and $460\%$.
%The gain is high in the other two finite-\ub scenarios too: avg $44\%$, with a maximum $85\%$ in the normal scenario, and avg $48\%$, with a maximum $114\%$ in the best.
As for infinite cap, \hybridalg yields avg gain over \johnson of $70\%$, $28\%$, and $30.6\%$ in the three scenarios.
%In some quarters the gain is even $133\%$.
%
The superiority of \hybridalg is confirmed over the other competitor, \bsalg: the avg gain is 
$139\%$, $ 45\%$, and $33\%$  in the finite-cap scenarios, and $37\%$, $16\%$, and $9\%$ in the infinite-cap cases, with max gain of $392\%$. % in the last quarter of the finite-\ub, worst scenario.
\emph{This attests the worthiness of employing the exact algorithm even only on small components.}
%In one quarter \bsalg and \hybridalg perform the same: the corresponding graph has no small components where the exact solution improves upon \bsalg.

% Comments about running time 1,86, 2,89 and 7,57
As far as running times, the fastest method is -- as expected -- the simplest \johnson.
%: in the finite-cap cases it takes on average $10s$. 
% ($1.9s$ in the worst scenario, $2.9s$ in the normal, and $7.6s$ in the best). 
The proposed \hybridalg takes from $3.5$s to $22$m, remaining perfectly compliant with the setting
of our RF service, which  runs  offline, at the end of each day. 
\hybridalg is comparable to \bsalg, due to the fact that the computation
on large components dominates. 
%On average, such a time is $11s$, $82s$, and $178s$ in the finite-\ub cases, and $216s$, $926s$, and $901s$ in the infinite-\ub scenarios.




% For bold fonts inside siunitx, use \bfseries
\begin{table*}[t]
\vspace{-4mm}
\begin{center}
{
\caption{{\footnotesize \label{tbl:experimental-results} Proposed \hybridalg algorithm  vs. the other methods devised in this work.}}
\vspace{-0.2cm}
\scriptsize
%\begin{tabular}{@{~}l|@{~}|l @{~}||@{~}S[table-format=10]@{~}S[table-format=3.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~} ||@{~}S[table-format=10]@{~}S[table-format=4.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~} ||@{~}S[table-format=10]@{~}S[table-format=3.1]@{~}S[table-format=3.1]@{~}S[table-format=4.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~}} 
% \multicolumn{1}{@{~}c||@{~}}{}  &  \multicolumn{1}{@{~}c@{~}||@{~}}{} & \multicolumn{4}{@{~}c||@{~}}{\textbf{\johnson}} & \multicolumn{4}{@{~}c||@{~}}{\textbf{\bsalg}} & \multicolumn{6}{@{~}c@{~}}{\textbf{\hybridalg}} \\
%\multicolumn{1}{@{~}c||@{~}}{\textbf{Cap $+$}} & \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Quarter}}} &   {\multirow{2}{*}{\textbf{Amount}}} &   \multicolumn{1}{@{~}c@{~}}{\textbf{Time}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}} &  \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Clients}}} & {\multirow{2}{*}{\textbf{Amount}}} &    \multicolumn{1}{@{~}c@{~}}{\textbf{Time)}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}}&  \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Clients}}} & {\multirow{2}{*}{\textbf{Amount}}} & \multicolumn{1}{@{~}c@{~}}{\textbf{\%Gain vs}}  &  \multicolumn{1}{@{~}c@{~is }}{\textbf{\%Gain vs}}  &   \multicolumn{1}{@{~}c@{~}}{\textbf{Time}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}} & {\multirow{2}{*}{\textbf{Clients}}} \\ 
%%\vspace{-0.1cm} \multicolumn{1}{@{ }c||@{ }}{\hybridalg} 
% \multicolumn{1}{@{~}c||@{~}}{\textbf{Scenario}}  & \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} &  \multicolumn{1}{c@{~}}{\textbf{(s)}}  & \multicolumn{1}{c@{~}}{\textbf{\-vables}}  &  \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} & \multicolumn{1}{c@{~}}{\textbf{(s)}}  & \multicolumn{1}{c@{~}}{\textbf{\-vables}}&  \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{\textbf{\textsf{S}-\textsc{bb-lb}}} & \multicolumn{1}{@{ }c@{ }}{\textbf{\textsf{S}-\textsc{beam}}} & \multicolumn{1}{c@{~}}{\textbf{(s)}}  &  \multicolumn{1}{c@{~}}{\textbf{\-vables}} & \\
\begin{tabular}{@{}c@{ }||@{}c@{ }||@{}S[table-format=11]@{}@{ }S[table-format=2.1]@{}S[table-format=5]@{}S[table-format=4]@{ }||@{}S[table-format=11]@{}@{ }S[table-format=4.2]@{}S[table-format=5]@{}S[table-format=4]@{ }||@{}S[table-format=11]@{}S[table-format=3.1]@{}S[table-format=3.1]@{}S[table-format=4.1]@{ }S[table-format=5]@{}S[table-format=4]@{}}
 \multicolumn{1}{@{}c@{ }||}{}  &  \multicolumn{1}{c@{ }||}{} & \multicolumn{4}{@{ }c@{ }||}{\textbf{\johnson}} & \multicolumn{4}{@{}c@{}||}{\textbf{\bsalg}} & \multicolumn{6}{@{}c@{}}{\textbf{\hybridalg}} \\
\multicolumn{1}{@{}c@{ }||}{\textbf{cap}} & \multicolumn{1}{@{ }c@{ }||}{\multirow{2}{*}{\textbf{quarter}}} &   {\multirow{2}{*}{\textbf{amount}}} &   \multicolumn{1}{@{ }c@{}}{\textbf{time}} &  \multicolumn{1}{@{ }c@{}}{\textbf{recei-}} &  \multicolumn{1}{@{ }c@{ }||}{\multirow{2}{*}{\textbf{clients}}} &    {\multirow{2}{*}{\textbf{amount}}} &   \multicolumn{1}{@{ }c@{}}{\textbf{time}} &  \multicolumn{1}{@{ }c@{}}{\textbf{recei-}} &  \multicolumn{1}{@{ }c@{ }||}{\multirow{2}{*}{\textbf{clients}}} & {\multirow{2}{*}{\textbf{amount}}} & \multicolumn{1}{@{}c@{ }}{\textbf{\%gain vs}}  &  \multicolumn{1}{@{}c@{ }}{\textbf{\%gain vs}}  &   \multicolumn{1}{@{}r@{ }}{\textbf{time}} &  \multicolumn{1}{c}{\textbf{recei-}} & {\multirow{2}{*}{\textbf{clients}}} \\ 
%\vspace{-0.1cm} \multicolumn{1}{@{ }c||@{ }}{\hybridalg} 
 \multicolumn{1}{@{}c@{ }||}{\textbf{scenario}}  & \multicolumn{1}{@{ }c@{ }||}{} &  &  \multicolumn{1}{r}{\textbf{(s)}}  & \multicolumn{1}{@{ }c@{}}{\textbf{\-vables}}  &  \multicolumn{1}{c||}{} &  &  \multicolumn{1}{r}{\textbf{(s)}}  & \multicolumn{1}{@{ }c@{}}{\textbf{\-vables}}  &  \multicolumn{1}{c||}{} &  \multicolumn{1}{c}{} &  \multicolumn{1}{@{}c@{ }}{\textbf{\textsf{S}-\textsc{bb-lb}}} & \multicolumn{1}{@{}c@{ }}{\textbf{\textsf{S}-\textsc{beam}}} & \multicolumn{1}{@{}r@{ }}{\textbf{(s)}}  &  \multicolumn{1}{c}{\textbf{\-vables}} & \\
\hline
{\multirow{4}{*}{\textbf{$<\!\!\infty$ W}}} & % {\multirow{6}{*}{\textbf{W}}} & 
$Q15_1$ & 95397950  & 1.8 & 1827 & 859 & 79014431   & 3.9 & 2532 & 939 & \bfseries 146703722	&  53.8 & 85.7 & 3.5 &  3330  & 1208 \\
 & $Q15_2$  & 121680562 &  1.8 & 1798 & 863 & 111184064  & 9.2 &  2222 & 891 & \bfseries 157007283	&  29.0 & 41.2 & 9.5 &  3263  & 1248 \\
  & $Q15_3$   & 52232665  & 1.9	 & 2066 & 987 & 59767431  & 14.4 &  2730 & 1034 & \bfseries 82875118	&  58.7 & 38.7 & 14.5 &  3619 & 1318 \\
 & $Q15_4$   & 46457493  &	 1.9	 & 1862 & 950 & 52872191  & 16.5 & 2499 & 987 & \bfseries 260196811 &  460.1  & 392.1 & 13.7 &  3296 & 1254 \\
 \hline
 {\multirow{4}{*}{\textbf{$<\!\!\infty$ N}}} & %\multirow{6}{*}{\textbf{N}}} &
$Q15_1$  & 162215076 &	2.7 &  4535  & 1986  & 146759007 & 99.1  & 6673  & 2269 & \bfseries 221401342 &  36.5 & 50.9 & 75.2  & 7951  &  2685 \\
 & $Q15_2$  & 151707991 & 2.8 &  4305  & 1975 & 133556473 & 47.5  & 5906  & 2141  & \bfseries 168556675 &  11.1 & 26.2 & 48.1  & 7080  &  2548 \\
 & $Q15_3$  & 143547779 &	3.0 &  5093  & 2200 & 158408830 & 76.2  & 7319  & 2464  & \bfseries 208011456 &  44.9 & 31.3 & 113.7 & 8172  &  2730 \\
 & $Q15_4$  & 149813738 &	 3.0 &  5137  & 2296 & 162254519 & 104.7  & 7459  & 2603 & \bfseries 277568569 &  85.3 & 71.1 & 117.5  & 8551  &  2941 \\
 \hline
 {\multirow{4}{*}{\textbf{$<\!\!\infty$ B}}} & %{\multirow{6}{*}{\textbf{B}}}& 
$Q15_1$   &  229604568	 & 7.6  &  7443  & 3115 & 263379260	& 172.1	& 11045	& 3566 & \bfseries 270221655 &  17.7	& 2.6 & 158.4 & 12004 & 3957	 \\
 & $Q15_2$  &  195171304	& 4.0  & 7183	 & 3108 & 208162233	& 133.6	& 10364	& 3506 & \bfseries 251353161 &  28.8	& 20.8 & 143.7 & 11669 & 3917	\\
 & $Q15_3$ 	&  236195806	 & 9.7  & 8397 & 3516 & 264654596	& 193.9	& 12564	& 4000 & \bfseries 314861548 &  33.3	& 19.0 & 205.4 & 13486 & 4333	\\
 & $Q15_4$ 	&  210056244	 & 8.9  & 9094 & 3801 & 234928905	& 212.5	& 13184	& 4259 & \bfseries 449862686 &  114.2	 & 91.5 & 239.3	 & 14360 & 4620 \\
 \hline
 \hline
 {\multirow{4}{*}{\textbf{$\infty$ W}}} & %{\multirow{6}{*}{\textbf{W}}} &  
$Q15_1$  & 194399317	 & 2.6 & 2863	 & 1275 &  215249395	 	& 110.4 & 5418	 & 1535	&  \bfseries 295595794	&  52.1 & 37.3 & 143.4 & 6528	 & 1872 \\	
 & $Q15_2$ 	&  215635790	 & 2.3 & 2939	 & 1283 &  263672222		& 124.5	 & 5285	 & 1490	&  \bfseries 319804764	&  48.3 & 21.3 & 125.2 & 6724	 & 1918 \\
 & $Q15_3$ 	&  206616203	 & 12.1 & 3329 & 1371 & 262778883		& 343.8	 & 6876	 & 1718	&  \bfseries 302740733	&  46.5 & 15.2 &  354.1 & 8290 & 2116 \\
 & $Q15_4$ 	& 216264862	 & 2.6 & 3224	 & 1383 &  286859858	 	& 287.3	 & 6034	 & 1685	&  \bfseries 504402450	&  133.2 & 75.8 &  304.9 & 7241 & 1992	\\
 \hline
 { \multirow{4}{*}{\textbf{$\infty$ N}}} & %{\multirow{6}{*}{\textbf{N}}} &
 $Q15_1$  & 553364544	 & 64.6	& 7131 & 2836	&  660907304	 	& 1168.9	 & 15323	& 3761	&  \bfseries 779733449	&   40.9	& 18.0 &  1006.2 &  17082	 & 4268	\\
 & $Q15_2$ 	& 643722123	 & 6.7 & 6742	 & 2736	&  663873349		& 619.0	& 14570	& 3507	&  \bfseries 784314578	&   21.8	& 18.1 &  690.1	 &  16761	& 4133	\\
 & $Q15_3$	& 693852990	& 29.0 & 7999 & 3034	&  743945529		& 1159.3	 & 17390	& 4143	&  \bfseries 827346450	&   19.2	& 11.2 &  1329.8 &  19544	 & 4701	\\
 & $Q15_4$ 	& 751368135	& 30.8 & 8289 & 3189	&  855932063	 	 & 757.8	 & 17666	&  4155	&  \bfseries 987866224	&   31.5	& 15.4 &  865.9	 &  19576	 & 4718	\\ 
 \hline
 { \multirow{4}{*}{\textbf{$\infty$ B}}} & %{\multirow{6}{*}{\textbf{B}} &
$Q15_1$  &  916036152	& 8.4	& 11246	& 4231 &  1110498564		& 866.0	& 23055	& 5353 & \bfseries 1172926462	&  28.0 & 5.6 &	 988.0	& 24811	& 5917	\\
 & $Q15_2$  &  1028777612	 & 26.3	& 10937	& 4159 &  1275000083		& 842.6	& 23235	& 5333 & \bfseries 1565296054	&  52.2 & 22.8 & 1182.7	& 25469	& 5901	\\
 & $Q15_3$ 	& 1329747599	 & 54.9	 & 13271	& 4830 &  \bfseries 1489713871		& 993.9	& 27404	& 6130  & \bfseries 1489713871 &  12.0 & 0 & 1101.0	& 27404	& 6130	\\
 & $Q15_4$  	& 1270225872	 & 22.1	& 13337	& 4835 &  1524865674		& 904.3	& 26177	& 5781 & \bfseries 1657784888 &  30.5 & 8.7 &  886.1	& 27746	& 6239	\\
\end{tabular}}
\end{center}
\vspace{-4mm}
\end{table*}



\begin{table}[t]
\vspace{-1mm}
\begin{center}
\scriptsize
\caption{\label{table:scalability}{\footnotesize Scalability of the proposed \hybridalg algorithm.}}
\vspace{-2mm}
\begin{tabular}{S[table-format=2]@{~}S[table-format=3]@{~~}S[table-format=3]@{~~}S[table-format=8]@{~}S[table-format=2]@{~}|S[table-format=2]@{~}S[table-format=4]@{~~}S[table-format=4]@{~~}S[table-format=9]@{~}S[table-format=5]}
{\bf days} & {\bf nodes} & {\bf arcs} & {\bf amount} & {\bf time} & {\bf days} & {\bf nodes} & {\bf arcs} & {\bf amount} & {\bf time} \\
\hline
%5 & 15983 & 14466 & 185959 & 1 & 30 & 106167 & 183570 & 16151068 & 65\\
%10 & 41088 & 43244 & 873317 & 4 & 60 & 143989 & 377635 & 38063145 & 3291 \\
%15 & 68183 & 85454 & 3471960 & 17 & 90 & 168861 & 600172 &  73101255 & 27504\\
5 & 15K & 14K & 185959 & 1 & 30 & 106K & 183K & 16151068 & 65\\
10 & 41K & 43K & 873317 & 4 & 60 & 143K & 377K & 38063145 & 3291 \\
15 & 68K & 85K & 3471960 & 17 & 90 & 168K & 600K &  73101255 & 27504\\
\hline
\vspace{-8mm}
\end{tabular}
\end{center}
\end{table}




\spara{Scalability.}
To test the scalability of \hybridalg, we randomly sampled segments of data corresponding 
to $5$, $10$, $15$, $30$, $60$, and $90$ days, collapsed the receivables of each segment into a single \bmultigraph, and ran \hybridalg on it, setting $\maxcyclelength \!=\! 10$ and $K \!=\!100$, and considering the finite-cap, normal scenario.
%The goal of this experiment was to assess the running time of \hybridalg on larger graphs. 
Table \ref{table:scalability} reports the outcome of this experiment, showing, for each segment, size of the \bmultigraph, settled amount, and running time.
As a side note, the amounts in Table~\ref{tbl:experimental-results} 
are generally larger than those reported here. 
The amounts of the two experiments are in fact not comparable, as Table~\ref{tbl:experimental-results} 
reports amounts summed over all time instants of a quarter, each expanded to a window of 5, 10 or 15 days depending on the \lifetime parameter.
For the same reason,  running time is instead comparable up to the 15-day segment. %, as the first table reports average per-day running time.
%Indeed, when up to $15$ days are considered, the achieved times are consistent with those reported before. 
Until $30$ days, the algorithm takes up to roughly a minute. 
The runtime increases on the two larger segments, becoming less than one hour and about $7.5$ hours, respectively. 
Albeit this increase is remarkable, we recall that network-based RF is designed to function offline, at the end of a working day.
In this setting even those larger times would be acceptable.
Moreover, as the service works on a daily basis, the realistic data sizes that \hybridalg has to handle are those of the previous experiment.
Finally, the tested implementation is sequential:  it can be improved by parallelizing it on the different connected components.
%. of the input multigraph.


% time intervals: Q1 =  2017-07/09, Q2 =  2017-10/12, Q3 =  2018-01/03 , Q4 = 2018-04/06 
%\begin{tabular}{l || S[table-format=5.1]@{ }@{ }S[table-format=5.1] | S[table-format=5.1]@{ }@{ }S[table-format=5.1]  || S[table-format=5.1]@{ }@{ }S[table-format=6.1] | S[table-format=5.1]@{ }@{ }S[table-format=6.1] || S[table-format=6.1]@{ }@{ }S[table-format=6.1] | S[table-format=6.1]@{ }@{ }S[table-format=6.1]} 
 %\multicolumn{1}{c}{\textbf{}}  & \multicolumn{4}{c}{\textbf{Worst Scenario}} & \multicolumn{4}{c}{\textbf{Normal Scenario}} & \multicolumn{4}{c}{\textbf{Best Scenario}} \\
%& \multicolumn{2}{c}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c||}{\textbf{CAP $= \infty$}} & \multicolumn{2}{c}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c||}{\textbf{CAP $= \infty$}} & \multicolumn{2}{c}{\textbf{CAP $ < \infty$}} & \multicolumn{2}{c}{\textbf{CAP $= \infty$}} \\
%&  \textbf{Avg} & \textbf{Max} &  \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max}  & \textbf{Avg} & \textbf{Max} & \textbf{Avg} & \textbf{Max }\\ 






%\begin{table*}[t]
%\vspace{-2mm}
%\begin{center}{
%\caption{\footnotesize \label{tbl:path-results} Algorithms adding paths between cycles}
%\vspace{-0.3cm}
%\scriptsize
%\begin{tabular}{ c c c  | S[table-format=4]   S[table-format=9]  | S[table-format=4]     S[table-format=9]   S[table-format=4]     | S[table-format=4]   S[table-format=9]     S[table-format=4]     S[table-format=2.1]     } 
%\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{} & \multicolumn{2}{|c}{\textbf{\hybridalg}} & \multicolumn{3}{|c}{\textbf{\pathalggreedy}} & \multicolumn{4}{|c}{\textbf{\pathalgsuk}} \\
%\multicolumn{1}{c}{\textbf{Cap}} & \multicolumn{1}{c}{\textbf{Scen-}} & \multicolumn{1}{c}{\textbf{Quar-}}  & \multicolumn{1}{|c}{\textbf{Avg}}  & \multicolumn{1}{c} {\multirow{3}{*}{\textbf{Amount}}} &  \multicolumn{1}{|c}{\textbf{Avg}}  &  {\multirow{3}{*}{\textbf{Amount}}} & \multicolumn{1}{c}{\textbf{\%Gain}}  &  \multicolumn{1}{|c}{\textbf{Avg}}  &  {\multirow{3}{*}{\textbf{Amount}}} & \multicolumn{1}{c}{\textbf{\%Gain}}  &  \multicolumn{1}{c}{\textbf{\%Gain}}  \\
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{ario}}  &  \multicolumn{1}{c}{\textbf{ter}} &   \multicolumn{1}{|c}{\textbf{Time}} & &  \multicolumn{1}{|c}{\textbf{Time}} & &  \multicolumn{1}{c}{\textbf{vs}}  &  \multicolumn{1}{|c}{\textbf{Time}} & &  \multicolumn{1}{c}{ \textbf{vs}} &   \multicolumn{1}{c}{\textbf{vs}}  \\ 
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{}  &  &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{c}{\hybridalg}  &  \multicolumn{1}{|c}{\textbf{(s)}} & &   \multicolumn{1}{c}{\pathalggreedy}  &   \multicolumn{1}{c}{\hybridalg} \\ 
%\hline
%{\multirow{12}{*}{\textbf{$<\!\!\infty$}}} & \textbf{W} &  $Q17_1$  & 4 & 208452169 & 4 & 206122369 & -1 &  54 & 208658217	& 1 & 0.1 \\
%& &    $Q17_2$  & 6 & 133998727 &  6 & 142880339 & 7 & 38 & 139157842	& -3 & 3.9   \\
%& &  $Q17_3$  & 5 & 250919555 & 4 & 251236654 & 0 & 18	& 251689885	& 0 & 0.3  \\
%& &   $Q17_4$  & 6 & 435864820 & 6 & 436866648 & 0 & 54	& 437305782	& 0 & 0.3  \\
%\cline{2-12}
%& \textbf{N} &   $Q17_1$  & 8 & 100052350 & 8 & 171073852 & 71 & 375 & 130166286 & -24 & 30.1  \\
%& &  $Q17_2$  & 95 & 210803336 & 47 & 224572822 & 7 & 525	& 222848364	& -1 & 5.7  \\
%&  &  $Q17_3$  & 13 &  181024199 & 14 & 187757266 & 4 & 429	& 215370572	&15 & 19.0  \\
%& &  $Q17_4$  & 23 & 405407829 & 38 & 425474537 & 5 & 448 & 413760885	& -3 & 2.1  \\
% \cline{2-12}
%& \textbf{B} &  $Q17_1$  & 50 & 128172168 &  47 & 139304792 & 9 & 576	& 140389844	& 1 & 9.5  \\
%&  &   $Q17_2$  & 215 & 223972720 & 185 & 238760149 & 7 & 721 & 245781771	& 3 & 9.7  \\
%&  & $Q17_3$  & 66 & 138227899 & 34 & 154369240 & 12 & 677	& 158211843 & 2 & 14.5 \\
%&  & $Q17_4$  & 192 & 380133762 & 109 & 395718595 & 4 & 1150 & 392670886 & -1 & 3.3  \\
%\hline
%\hline
%{\multirow{12}{*}{\textbf{$\infty$}}} & \textbf{W} &  $Q17_1$   & 20 & 374766629 &  7 & 401557792 & 7 &  256	& 407383061 & 1 & 8.7  \\
% & &  $Q17_2$  & 169 & 226076200 & 122 & 250268430 & 11 & 330	& 264854214 & 6 & 17.2  \\
%& & $Q17_3$  & 17 & 300021017 & 17 & 317522710 & 6 & 300 & 316476954	& 0 & 5.5  \\
%& &  $Q17_4$   & 98 & 516434249 & 101 & 540613736 & 5 & 214 & 543879376	& 1 & 5.3  \\
%\cline{2-12}
%& \textbf{N}  &  $Q17_1$  & 246 & 395904601 & 162 & 434561172 & 10 &  1761 & 458001083 & 5 & 15.7  \\
%&  & $Q17_2$  & 968 & 555117105 & 739 & 622621171 & 12 &   2023 & 624403545 & 0 & 12.5 \\
%&  &  $Q17_3$  & 573 & 471313548 & 505 & 516884575 & 10 &  1766 & 604594618 & 17 & 28.3  \\
%&  & $Q17_4$  & 884 & 679395059 & 694 & 713902252 & 5  & 2279 & 727907790 & 2 & 7.1  \\
% \cline{2-12}
%& \textbf{B} &  $Q17_1$  & 804 & 552458593 & 634 & 602544685 & 9 & 3004 & 538053935  & -11 & -2.6  \\
%&  & $Q17_2$  & 1604 & 699245106 & 1170 & 819639994 & 17 &  4822 & 727206932 & -11 & 4  \\
%& &  $Q17_3$  & 971 & 544101823 & 814 & 647240125 & 19 &  3430 & 685719252 & 6 & 26  \\
%&  & $Q17_4$  & 1609 & 907115932 & 943	& 970525923 & 7 &  3360 & 963608594	& -1 & 6.2  \\
%\end{tabular}}
%\end{center}
%\vspace{-4mm}
%\end{table*}

\begin{table*}[t]
\vspace{-2mm}
\begin{center}{
\caption{\footnotesize \label{tbl:path-results} Evaluating path selection: proposed \hybridalgp algorithm  vs. competitors.}
\vspace{-0.2cm}
\scriptsize
\begin{tabular}{ c c c  | S[table-format=4]   S[table-format=9]  | S[table-format=4]     S[table-format=9]   S[table-format=4]     | S[table-format=4]   S[table-format=9]     S[table-format=4]     S[table-format=2.1]     } 
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{} & \multicolumn{2}{|c}{\textbf{\hybridalg}} & \multicolumn{3}{|c}{\textbf{\pathalggreedy}} & \multicolumn{4}{|c}{\textbf{\pathalgsuk}} \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{cap}}} & \multicolumn{1}{c}{\textbf{scen-}} & \multicolumn{1}{c}{\textbf{quar-}}  & \multicolumn{1}{|c}{\textbf{time}}  & \multicolumn{1}{c} {\multirow{2}{*}{\textbf{amount}}} &  \multicolumn{1}{|c}{\textbf{time}}  &  {\multirow{2}{*}{\textbf{amount}}} & \multicolumn{1}{c}{\textbf{\%gain vs}}  &  \multicolumn{1}{|c}{\textbf{time}}  &  {\multirow{2}{*}{\textbf{amount}}} & \multicolumn{1}{c}{\textbf{\%gain vs}}  &  \multicolumn{1}{c}{\textbf{\%gain vs}}  \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{ario}}  &  \multicolumn{1}{c}{\textbf{ter}} &   \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{c}{\textbf{\hybridalg}}  &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{c}{ \textbf{\pathalggreedy}} &   \multicolumn{1}{c}{\textbf{\hybridalg}}  \\ 
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{}  &  &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{|c}{\textbf{(s)}} & &  \multicolumn{1}{c}{\hybridalg}  &  \multicolumn{1}{|c}{\textbf{(s)}} & &   \multicolumn{1}{c}{\pathalggreedy}  &   \multicolumn{1}{c}{\hybridalg} \\ 
\hline
{\multirow{12}{*}{\textbf{$<\!\!\infty$}}} & \multirow{4}{*}{\textbf{W}} &  $Q17_1$  & 4 & 208452169 & 4 & 206122369 & -1 &  54 & 208658217	& 1 & 0.1 \\
& &    $Q17_2$  & 6 & 133998727 &  6 & 142880339 & 7 & 38 & 139157842	& -3 & 3.9   \\
& &  $Q17_3$  & 5 & 250919555 & 4 & 251236654 & 0 & 18	& 251689885	& 0 & 0.3  \\
& &   $Q17_4$  & 6 & 435864820 & 6 & 436866648 & 0 & 54	& 437305782	& 0 & 0.3  \\
\cline{2-12}
& \multirow{4}{*}{\textbf{N}} &   $Q17_1$  & 8 & 100052350 & 8 & 171073852 & 71 & 375 & 130166286 & -24 & 30.1  \\
& &  $Q17_2$  & 95 & 210803336 & 47 & 224572822 & 7 & 525	& 222848364	& -1 & 5.7  \\
&  &  $Q17_3$  & 13 &  181024199 & 14 & 187757266 & 4 & 429	& 215370572	&15 & 19.0  \\
& &  $Q17_4$  & 23 & 405407829 & 38 & 425474537 & 5 & 448 & 413760885	& -3 & 2.1  \\
 \cline{2-12}
& \multirow{4}{*}{\textbf{B}} &  $Q17_1$  & 50 & 128172168 &  47 & 139304792 & 9 & 576	& 140389844	& 1 & 9.5  \\
&  &   $Q17_2$  & 215 & 223972720 & 185 & 238760149 & 7 & 721 & 245781771	& 3 & 9.7  \\
&  & $Q17_3$  & 66 & 138227899 & 34 & 154369240 & 12 & 677	& 158211843 & 2 & 14.5 \\
&  & $Q17_4$  & 192 & 380133762 & 109 & 395718595 & 4 & 1150 & 392670886 & -1 & 3.3  \\
\hline
\hline
{\multirow{12}{*}{\textbf{$\infty$}}} & \multirow{4}{*}{\textbf{W}} &  $Q17_1$   & 20 & 374766629 &  7 & 401557792 & 7 &  256	& 407383061 & 1 & 8.7  \\
 & &  $Q17_2$  & 169 & 226076200 & 122 & 250268430 & 11 & 330	& 264854214 & 6 & 17.2  \\
& & $Q17_3$  & 17 & 300021017 & 17 & 317522710 & 6 & 300 & 316476954	& 0 & 5.5  \\
& &  $Q17_4$   & 98 & 516434249 & 101 & 540613736 & 5 & 214 & 543879376	& 1 & 5.3  \\
\cline{2-12}
& \multirow{4}{*}{\textbf{N}}  &  $Q17_1$  & 246 & 395904601 & 162 & 434561172 & 10 &  1761 & 458001083 & 5 & 15.7  \\
&  & $Q17_2$  & 968 & 555117105 & 739 & 622621171 & 12 &   2023 & 624403545 & 0 & 12.5 \\
&  &  $Q17_3$  & 573 & 471313548 & 505 & 516884575 & 10 &  1766 & 604594618 & 17 & 28.3  \\
&  & $Q17_4$  & 884 & 679395059 & 694 & 713902252 & 5  & 2279 & 727907790 & 2 & 7.1  \\
 \cline{2-12}
& \multirow{4}{*}{\textbf{B}} &  $Q17_1$  & 804 & 552458593 & 634 & 602544685 & 9 & 3004 & 538053935  & -11 & -2.6  \\
&  & $Q17_2$  & 1604 & 699245106 & 1170 & 819639994 & 17 &  4822 & 727206932 & -11 & 4  \\
& &  $Q17_3$  & 971 & 544101823 & 814 & 647240125 & 19 &  3430 & 685719252 & 6 & 26  \\
&  & $Q17_4$  & 1609 & 907115932 & 943	& 970525923 & 7 &  3360 & 963608594	& -1 & 6.2  \\
\end{tabular}}
\end{center}
\vspace{-4mm}
\end{table*}








%\begin{table}[t]
%\vspace{-4mm}
%\begin{center}
%{
%\caption{{\footnotesize \label{tbl:experimental-results} Proposed \hybridalg algorithm  vs. competitors.}}
%\vspace{-0.2cm}
%\scriptsize
%%\begin{tabular}{@{~}l|@{~}|l @{~}||@{~}S[table-format=10]@{~}S[table-format=3.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~} ||@{~}S[table-format=10]@{~}S[table-format=4.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~} ||@{~}S[table-format=10]@{~}S[table-format=3.1]@{~}S[table-format=3.1]@{~}S[table-format=4.1]@{~}S[table-format=5]@{~}S[table-format=4]@{~}} 
%% \multicolumn{1}{@{~}c||@{~}}{}  &  \multicolumn{1}{@{~}c@{~}||@{~}}{} & \multicolumn{4}{@{~}c||@{~}}{\textbf{\johnson}} & \multicolumn{4}{@{~}c||@{~}}{\textbf{\bsalg}} & \multicolumn{6}{@{~}c@{~}}{\textbf{\hybridalg}} \\
%%\multicolumn{1}{@{~}c||@{~}}{\textbf{Cap $+$}} & \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Quarter}}} &   {\multirow{2}{*}{\textbf{Amount}}} &   \multicolumn{1}{@{~}c@{~}}{\textbf{Time}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}} &  \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Clients}}} & {\multirow{2}{*}{\textbf{Amount}}} &    \multicolumn{1}{@{~}c@{~}}{\textbf{Time)}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}}&  \multicolumn{1}{@{~}c||@{~}}{\multirow{2}{*}{\textbf{Clients}}} & {\multirow{2}{*}{\textbf{Amount}}} & \multicolumn{1}{@{~}c@{~}}{\textbf{\%Gain vs}}  &  \multicolumn{1}{@{~}c@{~is }}{\textbf{\%Gain vs}}  &   \multicolumn{1}{@{~}c@{~}}{\textbf{Time}} &  \multicolumn{1}{@{~}c@{~}}{\textbf{Recei-}} & {\multirow{2}{*}{\textbf{Clients}}} \\ 
%%%\vspace{-0.1cm} \multicolumn{1}{@{ }c||@{ }}{\hybridalg} 
%% \multicolumn{1}{@{~}c||@{~}}{\textbf{Scenario}}  & \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} &  \multicolumn{1}{c@{~}}{\textbf{(s)}}  & \multicolumn{1}{c@{~}}{\textbf{\-vables}}  &  \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} & \multicolumn{1}{c@{~}}{\textbf{(s)}}  & \multicolumn{1}{c@{~}}{\textbf{\-vables}}&  \multicolumn{1}{@{ }c||@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{} &  \multicolumn{1}{@{ }c@{ }}{\textbf{\textsf{S}-\textsc{bb-lb}}} & \multicolumn{1}{@{ }c@{ }}{\textbf{\textsf{S}-\textsc{beam}}} & \multicolumn{1}{c@{~}}{\textbf{(s)}}  &  \multicolumn{1}{c@{~}}{\textbf{\-vables}} & \\
%\begin{tabular}{@{}c@{ }||@{}c@{ }||@{}S[table-format=11]@{}@{ }S[table-format=2.1]@{}S[table-format=5]@{}S[table-format=4]@{ }||@{}S[table-format=11]@{}@{ }S[table-format=4.2]@{}S[table-format=5]@{}S[table-format=4]@{ }||@{}S[table-format=11]@{}S[table-format=3.1]@{}S[table-format=3.1]@{}S[table-format=4.1]@{}}
% \multicolumn{1}{@{}c@{ }||}{}  &  \multicolumn{1}{c@{ }||}{} & \multicolumn{2}{@{ }c@{ }||}{\textbf{\johnson}} & \multicolumn{2}{@{}c@{}||}{\textbf{\bsalg}} & \multicolumn{4}{@{}c@{}}{\textbf{\hybridalg}} \\
%\multicolumn{1}{@{}c@{ }||}{\textbf{cap}} & \multicolumn{1}{@{ }c@{ }||}{\multirow{2}{*}{\textbf{quarter}}} &   {\multirow{2}{*}{\textbf{amount}}} &   \multicolumn{1}{@{ }c@{ }||}{\textbf{time}}  &   {\multirow{2}{*}{\textbf{amount}}} &   \multicolumn{1}{@{ }c@{ }||}{\textbf{time}}   & {\multirow{2}{*}{\textbf{amount}}} & \multicolumn{1}{@{}c@{ }}{\textbf{\%gain vs}}  &  \multicolumn{1}{@{}c@{ }}{\textbf{\%gain vs}}  &   \multicolumn{1}{@{}r@{ }}{\textbf{time}} \\ 
%%\vspace{-0.1cm} \multicolumn{1}{@{ }c||@{ }}{\hybridalg} 
% \multicolumn{1}{@{}c@{ }||}{\textbf{scenario}}  & \multicolumn{1}{@{ }c@{ }||}{} &  &  \multicolumn{1}{c||}{\textbf{(s)}}  &  &  \multicolumn{1}{c||}{\textbf{(s)}}   &  \multicolumn{1}{c}{} &  \multicolumn{1}{@{}c@{ }}{\textbf{\textsf{S}-\textsc{bb-lb}}} & \multicolumn{1}{@{}c@{ }}{\textbf{\textsf{S}-\textsc{beam}}} & \multicolumn{1}{@{}r@{ }}{\textbf{(s)}}  \\
%\hline
%{\multirow{4}{*}{\textbf{$<\!\!\infty$ W}}} & % {\multirow{6}{*}{\textbf{W}}} & 
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
% \hline
% {\multirow{4}{*}{\textbf{$<\!\!\infty$ N}}} & %\multirow{6}{*}{\textbf{N}}} &
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
% \hline
% {\multirow{4}{*}{\textbf{$<\!\!\infty$ B}}} & %{\multirow{6}{*}{\textbf{B}}}& 
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
% \hline
% \hline
% {\multirow{4}{*}{\textbf{$\infty$ W}}} & %{\multirow{6}{*}{\textbf{W}}} &  
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
% \hline
% { \multirow{4}{*}{\textbf{$\infty$ N}}} & %{\multirow{6}{*}{\textbf{N}}} &
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
% \hline
% { \multirow{4}{*}{\textbf{$\infty$ B}}} & %{\multirow{6}{*}{\textbf{B}} &
%$Q17_1$  \\
% & $Q17_2$  \\
% & $Q17_3$ 	\\
% & $Q17_4$  	\\
%\end{tabular}}
%\end{center}
%\vspace{-4mm}
%\end{table}



\spara{Evaluating path selection.}
% Reference macros for the 4 algorithms that we are going to compare
% \rfbaseline The baseline suggested by the reviwer
% \hybridalg The final algorithm proposed in the previous version of the paper, without paths
% hybridalgpg Hybrid plus path enumeration and greedy selection
% hybridalgps Hybrid plus path enumeration and optimized suk selection 
%
% order of the columns HYBRID_NOPATHS  / \hybridalg ) avg tikme and amount 
% then HYBRID_GREEDY avg time, amount, gain wrt no_paths 
% next is hibrid suk avg time, amount, gain vs greedy gain vs no paths
% finally the baseline: AMOUNT	vs NOPATHS	vs HYBRID_SUK
A further experiment we carried out was on the impact of enriching a cycle-based solution by adding paths between cycles. 
We picked \hybridalg, which the previous assessment proved to be our best cycle-selection-based algorithm, and  compared it to its path-selection variants: 
\pathalggreedy , which performs a simple greedy path selection, and, \pathalgsuk, which employs the more refined selection method in Algorithm~\ref{alg:bsalg}.
Both variants are based on the outline in Algorithm~\ref{alg:pathalg} (Section~\ref{algo:paths}).
We run this evaluation on the \secondlog dataset, keeping the same settings as the previous experiments. 
Results are reported in Table~\ref{tbl:path-results}. 

%We maintained the same settings that were used in the previous experiment: for each scenario, we split the dataset in quarters. For each scenario/quarter pair and for each algorithm, we report total amount (euros) of the settled receivables, 
%average per-day running time (in seconds). We compare the algorithms in terms of total amount settled, reporting percentage gain of the various comparisons. 

%We start by observing that our first path-based algorithm, \pathalggreedy, beats our best no-path method, \hybridalg, in all tests but one, the \emph{worst} scenario with finite cap, where it achieves a small loss ($1\%$).
%The average gain with respect to \hybridalg is respectively $1.5\%$, $21.75\%$ and $8\%$ iin the finite-cap worst, normal, and best scenarios, and $7.25\%$, $9.25\%$, and $13\%$ in the infinite-cap worst, normal, and best case. 
%
%The second path-based algorithm, \pathalgsuk, also beats \hybridalg in all tests, attesting the goodness of the idea of adding paths to the cycle-based solutions. 
%Its average gain with respect to \hybridalg is respectively $1.15\%$, $14.22\%$, and $9.25\%$ in the finite-cap worst, normal, and best scenarios, and $9.175\%$, $15.9\%$, and $8.4\%$.
%
%However, using  Algorithm~\ref{alg:bsalg} to select a subset of enumerated paths does not seem to improve results much with respect to the greedy method: 
%\pathalgsuk is not able to improve the results of  \pathalggreedy in half of the tests. In the other half of cases, it does beat the greedy method, but it only achieves moderate amount gains (average $5\%$). 
%If we compare the two path-based algorithms in terms of running time, we notice that \pathalggreedy running times are always comparable to those of \hybridalg, and actually smaller in $75\%$ of cases.
%This may be due to the fact that adding paths to the daily solutions computed in each quarter causes the algorithm to work on smaller graphs in the following days. 
%The running times of \pathalgsuk are in all cases one order of magnitude larger by those of \pathalggreedy and \hybridalg. Thus \pathalgsuk achieves small improvements on \pathalggreedy, while requiring a much higher computational cost: for this reason we believe that \pathalggreedy is our winning path-based method. 

The main finding here is that our path-based algorithms outperform the best no-path method in all configurations (but one, where they however exhibit small losses, i.e., 1\% and 2.6\%).
\pathalggreedy achieves an average gain over \hybridalg of, respectively, $1.5\%$, $21.8\%$ and $8\%$ in the finite-cap worst, normal, and best scenarios, and $7.3\%$, $9.3\%$, and $13\%$ in the infinite-cap worst, normal, and best cases. 
Similarly, the average gain of \pathalgsuk over \hybridalg is, respectively, $1.2\%$, $14.2\%$, and $9.2\%$ in the finite-cap worst, normal, and best scenarios, and $9.2\%$, $15.9\%$, and $8.4\%$ in the infinite-cap worst, normal, and best cases.
\emph{This attests the relevance of the idea of adding paths to the cycle-based solutions}. 

The two path-selection strategies are comparable: 
\pathalgsuk wins in 12 configurations, with 5\% avg gain, while \pathalggreedy wins in 8 configurations, with 7\%~avg~gain.

As for running time, \pathalggreedy is  comparable to \hybridalg, and actually faster in $75\%$ of cases.
The motivation may be that adding paths to a daily solution causes the algorithm to work on smaller graphs in the next days.
As expected, \pathalgsuk is instead consistently slower than \pathalggreedy and \hybridalg (about one order of magnitude), due to its more sophisticated path-selection strategy. 



\begin{table}[t]
\vspace{-2mm}
\begin{center}{
\caption{\footnotesize \label{tbl:tmp_violations} Evaluating method for avoiding temporary constraint violation (algorithm: \hybridalg; $\ub <\infty$)}
\vspace{-0.1cm}
\scriptsize
\begin{tabular}{ @{}c  |  c@{}@{}S[table-format=8]  |  c@{}S[table-format=8]  |  c@{}@{}S[table-format=8]@{} } 
%\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{} & \multicolumn{1}{|c}{\textbf{\hybridalg}} \\
\multicolumn{1}{c|}{\textbf{quarter}} & \multicolumn{1}{c@{}}{\textbf{scenario}} & \multicolumn{1}{@{}c|}{\textbf{amount}} & \multicolumn{1}{c@{}}{\textbf{scenario}}   &  \multicolumn{1}{@{}c|} {\textbf{amount}}  & \multicolumn{1}{c@{ }}{\textbf{scenario}}   &  \multicolumn{1}{@{ }c} {\textbf{amount}} \\
%\multicolumn{1}{c|}{\textbf{ter}} & \multicolumn{1}{c}{\textbf{ario}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\textbf{ario}}   &  \multicolumn{1}{c|} {}  & \multicolumn{1}{c}{\textbf{ario}}   &  \multicolumn{1}{c} {} \\
\hline
 $Q17_1$  & \multirow{4}{*}{\textbf{W}} &  7836382 & \multirow{4}{*}{\textbf{N}}   & 9343124 & \multirow{4}{*}{ \textbf{B}}   &  7580671 \\
$Q17_2$. &   &  10821713   &  & 14344480 &   &  12949508 \\
$Q17_3$  &  &  11026866 &  &   16408195 &    &  26962726 \\
 $Q17_4$  &    & 18073953  &   &  22214050 &   &  24885106 \\
\end{tabular}}
\end{center}
\vspace{-4mm}
\end{table}



\spara{Avoiding temporary constraint violation.}
We also tested the performance of the proposed method for avoiding temporary constraint violation (Algorithm~\ref{alg:negbal}).
We run this experiment on the \secondlog dataset, by employing the \bsalg algorithm and considering the finite-cap scenario.
The results are reported in Table~\ref{tbl:tmp_violations}.
We observe that, although the settled amount is expectedly less than its counterpart where temporary constraint violation is not addressed, this amount remains reasonably large, i.e., in the order of 1M/10M euros.
